AndroidLab: Training and Systematic Benchmarking of Android Autonomous Agents

Autonomous agents have become increasingly important for interacting with the real world. Android agents, in particular, have been recently a frequently-mentioned interaction method. However, existing studies for training and evaluating Android agents lack systematic research on both open-source and closed-source models. In this work, we propose AndroidLab as a systematic Android agent framework. It includes an operation environment with different modalities, action space, and a reproducible benchmark. It supports both large language models (LLMs) and multimodal models (LMMs) in the same action space. AndroidLab benchmark includes predefined Android virtual devices and 138 tasks across nine apps built on these devices. By using the AndroidLab environment, we develop an Android Instruction dataset and train six open-source LLMs and LMMs, lifting the average success rates from 4.59% to 21.50% for LLMs and from 1.93% to 13.28% for LMMs. AndroidLab is open-sourced and publicly available at https://github.com/THUDM/Android-Lab.

==> table/multi-device.tex <==
\begin{table}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}clcccccccccc@{}}
\toprule
\textbf{Device} & \textbf{Model} & \textbf{Total} & \textbf{Bluecoins} & \textbf{Calendar} & \textbf{Cantook} & \textbf{Clock} & \textbf{Contacts} & \textbf{Maps.me} & \textbf{PiMusic} & \textbf{Setting} & \textbf{Zoom} \\ \midrule
\multirow{5}{*}{Pixel 3a}    & GPT-4o                & \textbf{21.48}  & 13.3               & \textbf{14.3}     & \textbf{33.3}    & 18.5           & \textbf{33.3} 
                              & 0.0             & 16.7             & 21.7             & \textbf{60.0} \\
                             & GPT-4-Vision-Preview  & 19.48           & \textbf{20.0}      & 14.3              & 16.7             & 18.5           & 6.7               & 6.7             & \textbf{25.0}    & \textbf{30.4}    & 40.0          \\
                             & Gemini-1.5-Pro        & 17.71           & 6.7                & 0.0               & 16.7             & \textbf{22.2}  & 13.3              & \textbf{13.3}   & 8.3              & 26.1             & 40.0          \\
                             & Gemini-1.0            & 12.16           & 0.0                & 0.0               & 16.7             & 11.1           & 13.3              & 0.0             & 8.3              & 26.1             & 20.0          \\
                             & Qwen-VL-Max           & 8.11            & 0.0                & 0.0               & 8.3              & 14.8           & 0.0               & 0.0             & 0.0              & 17.4             & 20.0          \\ \midrule
\multirow{5}{*}{Pixel 8 Pro} & GPT-4o                & \textbf{33.16}  & \textbf{13.3}      & \textbf{14.3}     & 33.3             & 25.9           & \textbf{40.0}                                  & \textbf{13.3}   & \textbf{41.7}    & \textbf{56.5}    & \textbf{40.0} \\
                             & GPT-4-Vision-Preview  & 30.36           & 13.3               & 7.1               & \textbf{50.0}    & \textbf{33.3}  & 40.0              & 0.0             & 25.0             & 43.5             & 20.0          \\
                             & Gemini-1.5-Pro        & 21.11           & 0.0                & 0.0               & 16.7             & 22.2           & 33.3              & 0.0             & 8.3              & 43.5             & 40.0          \\
                             & Gemini-1.0            & 15.53           & 0.0                & 0.0               & 41.7             & 22.2           & 13.3              & 0.0             & 0.0              & 26.1             & 0.0           \\
                             & Qwen-VL-Max           & 9.94            & 0.0                & 0.0               & 25.0             & 25.9           & 0.0               & 0.0             & 0.0              & 8.7              & 0.0           \\ \midrule
\multirow{5}{*}{Pixel Fold}  & GPT-4o                & \textbf{24.07}  & 0.0                & \textbf{7.1}      & \textbf{41.7}    & 37.0           & \textbf{46.7}                                  & 0.0             & \textbf{8.3}     & 17.4             & \textbf{40.0} \\
                             & GPT-4-Vision-Preview  & 19.80           & \textbf{6.7}       & 7.1               & 25.0             & \textbf{40.7}  & 13.3              & 0.0             & 8.3              & \textbf{21.7}    & 20.0          \\
                             & Gemini-1.5-Pro        & 14.06           & 0.0                & 0.0               & 33.3             & 25.9           & 20.0              & 0.0             & 0.0              & 13.0             & 0.0           \\
                             & Gemini-1.0            & 12.46           & 0.0                & 0.0               & 16.7             & 33.3           & 13.3              & 0.0             & 0.0              & 8.7              & 0.0           \\
                             & Qwen-VL-Max           & 6.65            & 0.0                & 0.0               & 8.3              & 22.2           & 0.0               & 0.0             & 0.0              & 4.3              & 0.0           \\
\bottomrule
\end{tabular}}
\end{table}

==> table/task-table-sub.tex <==
\begin{table}[]
\centering
\caption{\textbf{Examples of Android Eval Tasks.} The task will only be considered correct if all sub-goals are achieved.}
\label{tab:examples}
\begin{tabularx}{\textwidth}{@{}lll@{}}
\toprule
\textbf{APP} & \textbf{Task} & \textbf{Sub Goals} \\ \midrule

Bluecoins & 
\begin{tabular}[c]{@{}l@{}}
Record an income of 8000 CNY in the books, \\
and mark it as "salary".
\end{tabular} & 
\begin{tabular}[c]{@{}l@{}}
· type: income \\ 
· cash: 8000 CNY \\
· note: salary
\end{tabular} \\ 
\midrule


Calendar  &
\begin{tabular}[c]{@{}l@{}}
Edit the event with title "work", \\ 
change the time to be 7:00 PM.
\end{tabular} & 
\begin{tabular}[c]{@{}l@{}}
· title: work \\
· state: editing \\
· date: today \\
· time: 7 PM
\end{tabular} \\ 
\midrule



Clock & 
\begin{tabular}[c]{@{}l@{}}
I need set an 10:30PM clock every weekend, \\
and label it as "Watch Football Games".
\end{tabular} &
\begin{tabular}[c]{@{}l@{}}
· time: 10:30PM \\
· frequency: every weekend \\
· label: Watch Football Games
\end{tabular} \\ 
\midrule


PiMusic &
\begin{tabular}[c]{@{}l@{}}
Sort Pink Floyd's songs \\
by duration time in descending order.
\end{tabular} &
\begin{tabular}[c]{@{}l@{}}
· page: ARTISTS \\
· artist: Pink Floyd \\
· order: descending by duration

\end{tabular} \\

\arrayrulecolor{black}\bottomrule
\end{tabularx}
\end{table}



==> table/tokens.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{Average generation tokens of different modes. We used the LLaMA3 tokenizer for calculation. }
\begin{tabular}{@{}cc@{}}
\toprule
\textbf{Mode} & \#Average Generation Tokens \\ \midrule
IT            & 4.96                        \\
XML/SoM       & 23.56                       \\
ReAct         & 67.89                       \\
SeeAct        & 129.12                      \\ \bottomrule
\end{tabular}
\end{table}
